Measuring design compliance using neural language models -- an automotive case study

As the modern vehicle becomes more software-defined, it is beginning to take significant effort to avoid serious regression in software design. This is because automotive software architects rely largely upon manual review of code to spot deviations from specified design principles. Such an approach is both inefficient and prone to error. In recent days, neural language models pre-trained on source code are beginning to be used for automating a variety of programming tasks. In this work, we extend the application of such a Programming Language Model (PLM) to automate the assessment of design compliance. Using a PLM, we construct a system that assesses whether a set of query programs comply with Controller-Handler, a design pattern specified to ensure hardware abstraction in automotive control software. The assessment is based upon measuring whether the geometrical arrangement of query program embeddings, extracted from the PLM, aligns with that of a set of known implementations of the pattern. The level of alignment is then transformed into an interpretable measure of compliance. Using a controlled experiment, we demonstrate that our technique determines compliance with a precision of 92%. Also, using expert review to calibrate the automated assessment, we introduce a protocol to determine the nature of the violation, helping eventual refactoring. Results from this work indicate that neural language models can provide valuable assistance to human architects in assessing and fixing violations in automotive software design.

==> acmart-primary/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> acmart-primary/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.78.  Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.79.  Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.80.  New journals: DLT, FAC


==> dump-1 <==
outline:
Intro
Choosing a design pattern to study
Constructing a compliance assessment system
Experiments and results
Conclusion

The level of alignment is then converted into a measure that helps explain compliance in an interpretable manner.

Even if the process spares no effort in avoiding bad design, when working with complex software systems, achieving even reasonably good design can be a formidable challenge \cite{TANG2010614}.

That is, code -- when sufficiently well-written -- is quite capable of explaining a set of ideas to fellow human programmers while simultaneously being comprehensible to a machine that process it. 

Additionally, in software engineering communities with a strong tradition of design, ostensibly explanatory programming recipes that address recurring design problems are curated, codified, at times standardized, and further proliferated as design patterns \cite{10.5555/186897}.

The critical part is to define the interface between the controller and the handler. Since it should be possible to allocate the controller to an arbitrary ECU, its means of interacting with the handler cannot be based on the assumption that they are allocated to the same ECU. 

\begin{enumerate}[wide, labelindent=0pt]
    \item \emph{Dilution of the pattern} -- The CH pattern describes the relation between controllers and handlers. An actual controller or handler is certain to contain code that lies outside the scope of its design objectives. Hence, an architect will have to identify the essence of a CH relation in a larger context in order to assess it.
    
    \item \emph{Variations in implementation} -- The CH pattern is a high-level design pattern that lends itself to many implementation variants. Hence, an architect needs to assess whether a particular style of implementation is a legitimate representation of the pattern. \looseness=-1

    \vspace{1mm}
    \item \emph{Benchmark for assessment} -- The availability of an ideal implementation of the CH pattern, would obviously simplify the assessment process. However, it is practically difficult to identify the ideal case. While one may be able to construct the near-ideal case for a single application like roof hatch control, this ideal may not be suitable for a different application like passenger mirror control. On the other hand, an attempt to idealize across diverse applications like roof hatch or mirror control is likely to result in something excessively abstract and simplistic. Hence, during the assessment process, an architect has to rely on a subjective mental model of the pattern, which is not only difficult to explicitly state, but also affects the objectivity of the assessment.
\end{enumerate}

One program embedding $e_X$ is therefore of shape (8192, 1024), with the first dimension referring to number of tokens in each program and the second, the dimension of each token embedding.

This creates the risk that (1) a likely query drawn for testing is not a true instance of the pattern, and (2) questionable pairs end up weakening the average jointness benchmark $r$. One way to mitigate this risk could be to use expert review to eliminate instances that are not true pairs. Architecturally, however, we reason this to be difficult because tenets of the CH pattern are defined only at the SWC level and not at the program level. This means that the question if a pair $(c, h)$ from the product set is a true CH pair or not is difficult to answer. 

\begin{algorithm}
    \caption{Experiments for compliance assessment}
    \label{alg:experiments}    
    \SetKwInOut{Parameters}{Parameters}
    \SetKwProg{Fn}{Function}{:}{}
    \SetNoFillComment
    \begin{small}        
        \Parameters{PLMs $\mathcal{F}_A, \mathcal{F}_B, \mathcal{F}_C $, TAS corpus $\mathcal{P}$, the product set of known instances of CH pattern $\mathcal{V}^*$}
        \tcc{Refer to Procedure \ref{alg:compliance} for the definition of $\mathcal{S}$}
        \For {$f ~in \lbrack \mathcal{F}_A, ~\mathcal{F}_B, ~\mathcal{F}_C \rbrack$}{
            $K^+ = []$, $L^+ = []$, $K^- = []$, $L^- = []$\\
            \tcc{Assessing likely cases $P^+$}
            \textbf{for} $(c, h)$ in $\mathcal{V}^*$ \textbf{do}:\\
                \hspace{1em}$k, l = \mathcal{S}(c, h, f, V)$, $V = \mathcal{V}^* \setminus \{(c, h)\}$ \\
                \hspace{1em}$K^+$.append($k$), $L^+$.append($l$)\\

            \tcc{Assessing unlikely cases $P^-$}
            \textbf{for} $\_$ in range($|\mathcal{V}^*|$) \textbf{do}: \\
                \hspace{1em}$k, l = \mathcal{S}(X, Y, f, \mathcal{V})$, $X, Y \sim U(\mathcal{P} \setminus $ set($\mathcal{V}^*))$ \\
                \hspace{1em}$K^-$.append($k$), $L^-$.append($l$)\\
        }          
    \end{small}
\end{algorithm}

\begin{figure}[h]
    \centering
    \includegraphics[width=1.0\linewidth]{figs/parallelogram.png}
    \caption{If a PLM has perfectly understood the CH design pattern, then program embeddings of a pair of pattern instances should form a parallelogram. \textcolor{red}{Change examples}}
    \label{fig:parallelogram}
\end{figure}

We choose \emph{Controller-Handler}, which promotes hardware abstraction in automotive control systems, as the design pattern to study. We then assess its compliance in a corpus of code that implements control functionality for truck platforms of a major vehicle manufacturer.

Our work -- especially the controlled experiment to measure the quality of assessment -- can also be seen as a technique that evaluates the level of design knowledge in a PLM. From this perspective it relates closely to techniques that evaluate general PLM capabilities. For instance, \cite{DBLP:journals/corr/abs-2107-03374}, with its focus on synthesizing functionally correct code introduces methods and evaluation corpora specific to this purpose. Similarly, \cite{DBLP:conf/nips/RoziereLCL20}, which focuses on source-to-source translation, introduces necessary evaluation. A compilation of evaluation measures for several programming automation tasks is available in \cite{DBLP:journals/corr/abs-2102-04664}. In comparison, our work targets the aspect of design awareness and introduces a technique to measure it by analyzing the regularity of program embeddings.\looseness=-1

==> figs/table3.tex <==
\begin{table}[h]
    \centering
    \caption{Performance on the relationship challenge$^1$}
    \resizebox{85mm}{!}{
        \begin{threeparttable}
        \begin{tabular}{|l|l|l|l|l|l|l|l|}
            \hline
            \multirow{2}{*}{\textbf{Embedding}}       &
            \multirow{2}{*}{\textbf{Model}}           &
            \multicolumn{2}{c|}{~$\mathbf{{N_c=1}}$~} &
            \multicolumn{2}{c|}{~$\mathbf{{N_c=6}}$~} &
            \multicolumn{2}{c|}{~$\mathbf{N_c=8}$~}                                                                                                      \\ \cline{3-8}
            \rule{0pt}{3ex}
                                             &       & ~${r^{10}}$~ & ~${r^{-10}}$~ & ~${r^{10}}$~ & ~${r^{-10}}$~ & ~${r^{10}}$~ & ~${r^{-10}}$~ \\
            \hline
            \multirow{4}{*}{{\thead{Simple                                                                                                        \\ relationship}}}          & PLM-C
                                             & 0.298
                                             & 0.168
                                             & 0.204
                                             & 0.204
                                             & 0.248
                                             & 0.148

            \\
            \cline{2-8}
                                             & DLM-C
                                             & 0.290
                                             & 0.166
                                             & 0.314
                                             & 0.184
                                             & 0.254
                                             & 0.136
            \\
            \cline{2-8}
                                             & PLM-J
                                             & 0.240
                                             & 0.188
                                             & 0.324
                                             & 0.310
                                             & 0.348
                                             & 0.310
            \\
            \cline{2-8}
                                             & DLM-J
                                             & 0.212
                                             & 0.186
                                             & 0.330
                                             & 0.330
                                             & 0.374
                                             & 0.304
            \\
            \hline
            \multirow{4}{*}{{\thead{Average                                                                                                       \\ relationship}}}         & PLM-C
                                             & 0.370
                                             & 0.068
                                             & 0.520
                                             & 0.108
                                             & 0.518
                                             & 0.060
            \\
            \cline{2-8}
                                             & DLM-C
                                             & 0.366
                                             & 0.084
                                             & 0.536
                                             & 0.116
                                             & 0.574
                                             & 0.072
            \\
            \cline{2-8}
                                             & PLM-J
                                             & 0.200
                                             & 0.172
                                             & 0.336
                                             & 0.354
                                             & 0.450
                                             & 0.238
            \\
            \cline{2-8}
                                             & DLM-J
                                             & 0.236
                                             & 0.164
                                             & 0.360
                                             & 0.34
                                             & 0.436
                                             & 0.244
            \\
            \hline
        \end{tabular}
        \begin{tablenotes}[flushleft]\footnotesize
            \item[1] Using 117 instances of \texttt{Handler} and 356 instances \texttt{Adapter} respectively for the C and Java language models. Java model performance shown on the \texttt{Adaptee} $\rightarrow$ \texttt{Client} relationship
        \end{tablenotes}
    \end{threeparttable}    
    }
    \label{table:relationship}
\end{table}


==> tables/2-vocab.tex <==
\begin{table}[t!]
    \caption{Mean accuracy $u^1$ on the vocabulary challenge$^2$}
    \centering
    \resizebox{85mm}{!}{
        \begin{threeparttable}
        \begin{tabular}{|l|l|l|l|l|l|}
            \hline
            \multirow{2}{*}{\textbf{Model}}         &
            \multirow{2}{*}{~$\mathbf{{u_B}}$~}     &
            \multirow{2}{*}{~$\mathbf{{u_O}}$~}     &
            \multicolumn{2}{c|}{~$\mathbf{{u_S}}$~} &
            \multirow{2}{*}{\textbf{BERT}~$\mathbf{{u_S}}$~}                                                                                         \\
            \cline{4-5}
            \rule{0pt}{3ex}
                                                    &                &  & ~$\mathbf{{L_c=512}}$~ & ~$\mathbf{{L_c=1024}}$~ & ($\mathbf{{L_c=1024}}$) \\
            \hline
            PLM-C
                                                    & 0.97
                                                    & 0.88
                                                    & 0.67 $\pm$ 0.2
                                                    & 0.74 $\pm$ 0.2
                                                    & 0.88
            \\
            \hline
            DLM-C
                                                    & 0.99
                                                    & 0.95
                                                    & 0.82 $\pm$ 0.1
                                                    & 0.87 $\pm$ 0.1
                                                    & 0.94
            \\
            \hline
            PLM-J
                                                    & 0.98
                                                    & 0.84
                                                    & 0.67 $\pm$ 0.2
                                                    & 0.71 $\pm$ 0.2
                                                    & 0.84
            \\
            \hline
            DLM-J
                                                    & 0.98
                                                    & 0.86
                                                    & 0.74 $\pm$ 0.1
                                                    & 0.76 $\pm$ 0.1
                                                    & 0.89

            \\
            \hline
        \end{tabular}
        \begin{tablenotes}[flushleft]\footnotesize
            \item[1] Divided by category B-Basic, O-Others, S-Special
            \item[2] 30\% of TAS and P-MARt used to challenge models of corresponding language            
        \end{tablenotes}
    \end{threeparttable}    
    }
    \label{table:vocab}
\end{table}


==> tables/3-vocab-corr.tex <==
\begin{table}[ht!]
    \caption{Correlation$^1$ of the accuracy of predicting design keywords ($u_S$) with key test factors$^2$}
    \centering

    \begin{threeparttable}
        \begin{tabular}{|l|l|l|l|l|}
            \hline
            \multirow{1}{*}{\textbf{Model}}        &
            \multirow{1}{*}{~$\mathbf{{L_c}}$~}    &
            \multirow{1}{*}{~$\mathbf{{M_s}}$~}    &
            \multirow{1}{*}{~$\mathbf{{u_{BO}}}$~} &
            \multirow{1}{*}{~$\mathbf{{M_{BO}}}$~}         \\
            \hline
            \multirow{2}{*}{PLM-C
            }
                                                   & 512
                                                   & -0.79
                                                   & 0.09
                                                   & -0.07
            \\
            \cline{2-5}
                                                   & 1024
                                                   & -0.77
                                                   & 0.09
                                                   & -0.07
            \\
            \hline
            \multirow{2}{*}{DLM-C
            }
                                                   & 512
                                                   & -0.72
                                                   & 0.17
                                                   & -0.14
            \\
            \cline{2-5}
                                                   & 1024
                                                   & -0.70
                                                   & 0.16
                                                   & -0.13
            \\
            \hline
            \multirow{2}{*}{PLM-J
            }
                                                   & 512
                                                   & -0.79
                                                   & 0.10
                                                   & -0.10
            \\
            \cline{2-5}
                                                   & 1024
                                                   & -0.74
                                                   & 0.12
                                                   & -0.11
            \\
            \hline
            \multirow{2}{*}{DLM-J
            }
                                                   & 512
                                                   & -0.78
                                                   & 0.20
                                                   & -0.19
            \\
            \cline{2-5}
                                                   & 1024
                                                   & -0.75
                                                   & 0.21
                                                   & -0.20
            \\
            \hline
        \end{tabular}
        \begin{tablenotes}[flushleft]\footnotesize
            \item[1] Pearson correlation coefficient
            \item[2] $L_c$: length of code snippet, $M_S$: foreground masking rate, $M_{BO}$: background masking rate, $u_{BO}$: background prediction accuracy
        \end{tablenotes}
    \end{threeparttable}

    \label{table:vocab-corr}
\end{table}


==> tables/4-relationships.tex <==
\begin{table}[h]
    \centering
    \caption{Performance on the relationship challenge$^1$}
    \resizebox{85mm}{!}{
        \begin{threeparttable}
        \begin{tabular}{|l|l|l|l|l|l|l|l|}
            \hline
            \multirow{2}{*}{\textbf{Embedding}}       &
            \multirow{2}{*}{\textbf{Model}}           &
            \multicolumn{2}{c|}{~$\mathbf{{N_c=1}}$~} &
            \multicolumn{2}{c|}{~$\mathbf{{N_c=6}}$~} &
            \multicolumn{2}{c|}{~$\mathbf{N_c=8}$~}                                                                                                      \\ \cline{3-8}
            \rule{0pt}{3ex}
                                             &       & ~${r^{10}}$~ & ~${r^{-10}}$~ & ~${r^{10}}$~ & ~${r^{-10}}$~ & ~${r^{10}}$~ & ~${r^{-10}}$~ \\
            \hline
            \multirow{4}{*}{{\thead{Simple                                                                                                        \\ relationship}}}          & PLM-C
                                             & 0.30
                                             & 0.17
                                             & 0.20
                                             & 0.20
                                             & 0.25
                                             & 0.15

            \\
            \cline{2-8}
                                             & DLM-C
                                             & 0.30
                                             & 0.17
                                             & 0.31
                                             & 0.19
                                             & 0.25
                                             & 0.14
            \\
            \cline{2-8}
                                             & PLM-J
                                             & 0.24
                                             & 0.19
                                             & 0.32
                                             & 0.31
                                             & 0.35
                                             & 0.31
            \\
            \cline{2-8}
                                             & DLM-J
                                             & 0.21
                                             & 0.19
                                             & 0.33
                                             & 0.33
                                             & 0.37
                                             & 0.30
            \\
            \hline
            \multirow{4}{*}{{\thead{Average                                                                                                       \\ relationship}}}         & PLM-C
                                             & 0.37
                                             & 0.07
                                             & 0.52
                                             & 0.11
                                             & 0.52
                                             & 0.06
            \\
            \cline{2-8}
                                             & DLM-C
                                             & 0.37
                                             & 0.09
                                             & 0.53
                                             & 0.12
                                             & 0.57
                                             & 0.07
            \\
            \cline{2-8}
                                             & PLM-J
                                             & 0.20
                                             & 0.17
                                             & 0.34
                                             & 0.35
                                             & 0.45
                                             & 0.24
            \\
            \cline{2-8}
                                             & DLM-J
                                             & 0.24
                                             & 0.16
                                             & 0.36
                                             & 0.34
                                             & 0.44
                                             & 0.24
            \\
            \hline
        \end{tabular}
        \begin{tablenotes}[flushleft]\footnotesize
            \item[1] Using 117 instances of \texttt{Handler} and 356 instances \texttt{Adapter} respectively for the C and Java language models. Java model performance shown on the \texttt{Adaptee} $\rightarrow$ \texttt{Client} relationship
        \end{tablenotes}
    \end{threeparttable}    
    }
    \label{table:relationship}
\end{table}

